High Accuracy and High Fidelity Extraction of Neural Networks

In a model extraction attack, an adversary steals a copy of a remotely deployed machine learning model, given oracle prediction access. We taxonomize model extraction attacks around two objectives: *accuracy*, i.e., performing well on the underlying learning task, and *fidelity*, i.e., matching the predictions of the remote victim classifier on any input. To extract a high-accuracy model, we develop a learning-based attack exploiting the victim to supervise the training of an extracted model. Through analytical and empirical arguments, we then explain the inherent limitations that prevent any learning-based strategy from extracting a truly high-fidelity model---i.e., extracting a functionally-equivalent model whose predictions are identical to those of the victim model on all possible inputs. Addressing these limitations, we expand on prior work to develop the first practical functionally-equivalent extraction attack for direct extraction (i.e., without training) of a model's weights. We perform experiments both on academic datasets and a state-of-the-art image classifier trained with 1 billion proprietary images. In addition to broadening the scope of model extraction research, our work demonstrates the practicality of model extraction attacks against production-grade systems.

==> diff_stability.tex <==
\subsection{Robustness of Differential Model Analysis}
In this section, we discuss the various improvements needed to make differential model analysis a practical algorithm to run in the presence of floating point imprecision.

\subsubsection{Failures Happen}
Causes for failure to measure weights:
\begin{itemize}
    \item Small weights make division blow up and give unreasonable values
    \item Small perturbations for finite differences give numerically unstable results
    \item Not going all the way out misses some neurons
\end{itemize}

\subsubsection{Getting around these failures}
\begin{itemize}
    \item Small weights: measure in different basis or ignore
    \item Run many search phases and compute l0 sparsity based connected components
\end{itemize}

\subsubsection{Making things work at depth}
Various tricks for making the algorithm work for deeper networks
\begin{itemize}
    \item Uncorrelated errors allow us to filter out the bad weights
    \item Before and after is just a linear transformation, so it can still be divided out in deeper layers
    \item Arbitrary basis + masked basis allow recovery even without control of input direction
\end{itemize}


==> future_work.tex <==
Future work/open problems:
\begin{enumerate}
    \item unknown label set/feature set
    \item how can we remove the unlabeled data assumption?
    \item how can we leverage the connection between fidelity and bayesian ML to improve/understand/predict our mistakes
    \item connection between defenses, accuracy, and fidelity - what can a defense do and what can't it
    \item make DNA better duh
\end{enumerate}

